MARS: Nano-Power Battery-free Wireless Interfaces for Touch, Swipe and Speech Input

Augmenting everyday surfaces with interaction sensing capability that is maintenance-free, low-cost (about $1), and in an appropriate form factor is a challenge with current technologies. MARS (Multi-channel Ambiently-powered Realtime Sensing) enables battery-free sensing and wireless communication of touch, swipe, and speech interactions by combining a nanowatt programmable oscillator with frequency-shifted analog backscatter communication. A zero-threshold voltage field-effect transistor (FET) is used to create an oscillator with a low startup voltage (about 500 mV) and current (< 2uA), whose frequency can be affected through changes in inductance or capacitance from the user interactions. Multiple MARS systems can operate in the same environment by tuning each oscillator circuit to a different frequency range. The nanowatt power budget allows the system to be powered directly through ambient energy sources like photodiodes or thermoelectric generators. We differentiate MARS from previous systems based on power requirements, cost, and part count and explore different interaction and activity sensing scenarios suitable for indoor environments.

==> notes.tex <==
MARS System Architecture consisting of Transmitter, Receiver and multiple MARS tags in the environment. Transmitter produces UHF RF Non-modulated continuous carrier wave (yellow) which is incident on the tags. Each MARS tag consists of an ultra-low-power oscillator, oscillating at a particular frequency ( e.g., Tag 1 oscillates at F1 frequency). The input interactions result in change in electrical property (blue) resulting in frequency modulating the oscillator signal (magenta). This signal is backscattered  to the receiver (green) using analog impedance switch and antenna. The receiver, receives frequency modulated information at different bands from each tag which is demodulated back to the original sensed signal.




The last decade has been use of backscatter communication as a technique to 


A recent wave of backscatter communication 
-- one which are batteryfree and look at form factor lack rich set of input possibilities or allowing multiple tags operating. 

%% NOTE : WE need to ack backscatter, active RFID, chipless RFID based interaction and then move to say its limitations in few lines before saying need for generalised architecture. 
Initial attempts at building such battery-free sensing systems pertained to expansion of energy harvesting to ambient room light and RF. While harvesting from ambient can be a viable approach, since operable power even after duty-cycling for active communication was still too high the systems could only operate using big solar cell would have to be installed or the distance of operation from RF source would be very less , effecting  

A recent wave of battery-free sensing systems optimizes power by shifting the digital tasks to the receiver and keeping the tag as a purely
analogue system with cleverly designed encoding schemes to communicate the information reliably to a receiver. Such systems consume power on the order of 100 microWatt [26, 35, 43]

Several systems based on backscatter communication have been recentrly been explored which have brought the power requirements to near 50 microWatt.  

battery-free flexible form factor touch sensing technologies based on Radio Frequency IDentification (RFID) like  PaperID\cite{}, RIO \cite{}, etc   
-- power is too high to be easily powered thus form factor is not good. 



Researchers have investigated  
Ambient power like solar, thermal 

To over come these, current work on based on RFID and backscatter based communication,  where the power consumeing  


 

\subsection{Battery-free Interaction Sensing} % 
	%Backscatter Communication:
	power , power harvestor form factor 
	
	ID:
	
	Touch:
    chipless sensors 
	RFID touch: 
	https://dl.acm.org/doi/abs/10.1145/2858036.2858249
	https://dl.acm.org/doi/10.1145/3332165.3347907
	
	
	RFID gesture:  
	https://dl.acm.org/doi/10.1145/3117811.3117818 
	https://dl.acm.org/doi/abs/10.1145/3117811.3117818
	ubiquitouch 
	%photodiode -- not solar panel.
     %%ambient environment.  
	
	sound 
	
	
    Backscatter Communication
	https://ieeexplore.ieee.org/abstract/document/8368232 
	
	
\subsection{Object based Interaction sensing} %form factor, 
    	
	
	
	\subsection{Low Voltage (LV) designs  }
	%Low POWER DESIGN METHODS/ 
	Sub-threshold Design for Ultra Low-Power Systems ---- Analog Integrated Circuits Design for Processing Physiological Signals 
	
     https://www.sciencedirect.com/science/article/pii/S0026269205003526 
     
     LOW-VOLTAGE LOW-POWER ANALOG CIRCUIT DESIGN
   











%$\omega_{0}^{2} L_{1} C_{eq} = 1$

%$C_{eq} = \frac{{\left( {C_{1} + C_{2} } \right)\frac{{L_{2} }}{{L_{1} }} + C_{1} - \sqrt {\left[ {\left( {C_{1} + C_{2} } \right)\frac{{L_{2} }}{{L_{1} }} - C_{1} } \right]^{2} + 4\frac{{L_{2} }}{{L_{1} }}C_{1}^{2} } }}{2}$

%ESCO with high swing for low supply voltages the value of a must be chosen relatively close to unity, which is achieved when C 2/C 1 ≪ 1. 

%$a_{{C_{2} \ll C_{1} }} = 1 + \frac{{{{C_{2} } \mathord{\left/ {\vphantom {{C_{2} } {C_{1} }}} \right. \kern-0pt} {C_{1} }}}}{{1 + {{L_{1} } \mathord{\left/ {\vphantom {{L_{1} } {L_{2} }}} \right. \kern-0pt} {L_{2} }}}}.$


% In this paper, a low voltage of a chaotic Colpitts oscillator is proposed. The proposed implementation of EPAD MOSFETs technology [5] adds functionality to the classical Chaos Colpitts Oscillator idea that operated in very low supply voltages. The second benefit from the EPAD MOSFETs is the employment of a floating gate structure, which can be precise, trimmed to produce tightly controlled transistor electrical characteristics. This is a very important feature, because a basic disadvantage of the analogue chaotic systems is the tolerance to the electrical characteristics that the analogue components, especially the active ones (transistors), appear. As a result of this, is the output difference of identical systems and the impossibility of synchronisation.

\subsection{Key ideas for System Design}

\subsubsection*{Reduction in operational power}
We have decreased the operational power budget required for sensing and communicating data by almost 2 orders of magnitude than previously reported in the literature (50 micro-Watt)  


\begin{enumerate}
\item\textbf{Shift of complex power consuming circuitry to a central Receiver Hub :} Backscatter communication  \cite{}
FSk--simultaneosu, simultaneous operation of multiple tags 
A recent wave of battery-free sensing systems optimizes power by shifting the digital tasks to the receiver and keeping the tag as a purely analogue system with cleverly designed encoding schemes to communicate the information reliably to a receiver. 


\item\textbf{Reduction in Operational Power of tag by use of oscillator operated in sub-threshold region:} 
The fundamental and also the most power consuming component in frequency shift keying based backscatter communication is an oscillator as it modulates the frequency based on the sensed phenomenon. We have built an oscillator which operates in sub-threshold mode \cite{} reducing oscillator power budget to just few 100s of nanoWatt with an extremely low startup voltage $\sim$ \startupVoltage mV. 
	
%This modulates the frequency based on the sensed phenomenon which is recived a.Voltage controlled Oscillator: presence , Capacitor controlled Oscillator

\item\textbf{Depletion Mode FET as RF-switch to compliment subthreshold region oscillator :}  
To compliment the low-voltage frequency modulated outputs (~20mV) from the the oscillator a depletion Mode FET  which is employed as RF-switch as it is on Vgs=0 

combined circuit can operate in low voltage, no PM, many harvestors in-situ ambient environemnt, 


\item\textbf{Flexibility of combined system} 

\item \textbf{Use of Miller effect of FET for combined sensing and power harvesting:} 

ID, 

\item \textbf{ Use of variable capacitance for Controlling sub-threshold oscillator:} 
sensing : touch, 

\end{enumerate}

Such drastic reduction in power and startup voltage, has allowed us to be creative with the number and kinds of power harvestors which we can use. While generally power harvested from 


\subsection*{Push for Power Harvestors with thin and small in Form factor}
Secondly, we have used harvesting devices and self-powered sensors which showed the promise of being less in component size, thin in form factor while still being able to provide the power required for operation.
6. Expansion of harvesting space : 
Match harvestors for easy interactions 













Early in the development of the MOS technology it became clear that the reduction of the supply voltage was
a prerequisite for circuit miniaturization and power reduction\cite{macii2004ultra}. While the supply voltage decreases the threshold Voltage does not scale in equal proportion\cite{macii2004ultra}





%============================================
%============================================
%============================================
%MORE RANDOM TEXT ================================


%Today, our ambient indoor environment consists of various kinds of power sources \cite{}, scattered all around us in different scales of magnitude (nW to W)\cite{}. 

% light on an object , practically use small space. x+object=object. 

%1. activity > interaction 
%2. [ context sensing, input controls]
%3. sensors are externally powered. 
%4. recently self-sustainable sensing but they usually use high and medium intensity activities have been used--- write reasons which 
%5. Low activities sensing ignored -- 
%a.Consumption -- appropriate system architecture not approporiated makde which can detect such low power activities since communication is >>> power than harvested 
%b. Generation -- "micro-interaction power harvesting we need proper form factor of harvetsors is VERY imp."  --  micro-interaction 




4. While we want to do that we also want this data collection to be hassle free therforere wireless sensing nodes and self-sustainability. 
 
 For true ubiquitous sensing, these nodes should be embedded in everyday objects and surfaces without being a hindrance in for the object's functional usage or aesthetics and, self-sustainable to avoid constant battery maintenance effort and toxic battery waste. This is a hard research problem.
 
 self-sustainable to avoid constant battery maintenance effort and toxic battery waste. This is a hard research problem 
 
 
 6. self-sustainbility is hard --- The real power harvested from these activities can depends on multiple factors the energy harvesting device and circuit used which usually 1-10\% efficiency reducing power to sub-microwatt.  %%now add form factor 
 
 
 7. While extensive research has been done on sensing of high and medium intensity activities , it is the low-power activities which are hard to sense. 
 
 3. This power can be utilised for a dual operation of both a energy source or source of information ; 
 in addition to the obvious energy source it carries information about human activities and infrastructure usages which can be leveraged for context sensing and input control applications \cite{}.






5. While there has been extensive research done on building sensing solutions for high and medium power intensity activities 



5. places where micro-interaction low power activities are used are objects, there major factor is not chnaging the shape/functionality of the object. thus only 



Extensive research has been done on building sensing and power technologies for all the three types of intensity.  , where it was evident that only 10-30\% of power from the original mechanical interaction can be harvested



Humans are mobile sources of energy \cite{}. Everyday human activities dissipate energy from the human body into the physical surface being interacted with -- high intensity mobile activities (10W) e.g. running release energy into the floor, medium energy (1W) e.g. walking, sitting up releases energy into shoes or sofa respectively 
, and low-power implicit activities like touch, sliding of hand


Our ambient environment consists of a spectrum of power sources differentiated by the type of physical phenomenon, magnitude of intensity (nanoWatt to Watt), and time duration (few seconds to hours long). 

These can be concentrated near an electrical appliance (e.g., mechanical, thermal, EM) \cite{}, omnipresent in the form of electromagnetic waves (e.g., light, RF waves) \cite{}, or generated in-situ due to human interactions (mechanical)\cite{} or  presence itself (thermal) \cite{}. 

1 photodiode 500nW of power 
2 photo.     1uW


These power sources have dual operation; in addition to being energy source they also carry information about human activities and infrastructure usages which can be leveraged for context sensing and input control applications \cite{}. 

With blurring of our digital and physical lives, constant research push for gathering 
granular data for context sensing and input control applications. 

With blurring of our digital and physical lives, there has been a constant focus on finding creative ways for deployment of sensing nodes in our everyday environment to gather granular data for context sensing and input control applications. 


For true ubiquitous sensing, these nodes should be embedded in everyday objects and surfaces without being a hindrance in for the object's funcational usage or aesthetics and, self-sustainable to avoid constant battery maintenance effort and toxic battery waste. This is a hard research problem.




With blurring of our digital and physical lives, researchers have focused on finding creative ways for building and deploying sensing nodes to gather granular data about everyday environment.  

While practical usage of these power sources as operational energy source for a circuit is dependent on multiple factors including their magnitude, duration, harvesting device and the power management circuit used, their fluctuations almost always can be used as a source of information about human activities and infrastructure usages. 


%These can be concentrated near an electrical appliance (e.g., mechanical, thermal, EM) \cite{}, omnipresent in the form of electromagnetic waves (e.g., light, RF waves) \cite{}, or generated in-situ due to human interactions (mechanical)\cite{} or  presence itself (thermal) \cite{}.

%These power sources have dual operation; in addition to being energy source they also carry information about human activities and infrastructure usages which can be leveraged for context sensing and input control applications \cite{}. 

Blurring of our digital and physical lives \cite{}, has lead to the rise in the demand for granular information \cite{} about everyday environment. researchers have focused on finding creative ways for deploying sensing nodes in the environment leveraging different types of power sources for both sensing and energy harvesting. 

 

Critical factor for self-sustainable system operation is that the input power harvested from the ambient sources should be more or equal to the power required for their functional operation. Till now this has been mostly been demonstrated for power sources sufficient high in intensity (e.g. jumping, walking, fire furnace) or prolonged in duration (e.g., mixer). so as to generate mw-W automatically excluding power source is low and short in magnitude (sub-microwatt) e.g., finger touch, hand sliding motion. 

In this paper we leverage power sources which are in-situ like humans or omnipresent like light, but without 


For true ubiquitous sensing, these nodes should be embedded in everyday objects and surfaces without being an obstacle for the object's usage or aesthetics and, self-sustainable to avoid constant battery maintenance effort and toxic battery waste. This is a hard research problem.

%These nodes often leverage ambient power sources to sense information about the physical space and if its magnitude and duration is sufficient then to even power their operation. 







%This requires the hardware system to be embedded in everyday objects and surfaces without being an obstacle for its usage or aesthetics and self-sustainable to avoid constant battery maintenance effort and toxic battery waste. 

This is mostly limited to  high (100mW-W e.g, ) and medium intensity activities (mW-100uW e.g, ) while low-power activities 



This paper looks at building appropriate wireless sensing architecture for sub-microwatt power budget activity detection. 

%


Continuous real-time self-sustainable operation of wireless sensing nodes has been achieved where ambient power source of high intensity (10mW-W) are present (e.g., mobile vibration environments like human running (mechanical), electrical equipment which get heated up to high temperatures (thermal)) and asynchronous self-sustainable operation 

the power source is present for long duration that the system can be duty-cycled to the point where enough operational power is harvested, self-sustainable operation becomes increasingly hard where power source is low and short in magnitude (sub-microwatt) e.g., finger touch, hand sliding motion. 

For true ubiquity, these nodes should be embedded in everyday objects and surfaces without being an obstacle for the object's usage or aesthetics and, self-sustainable to avoid constant battery maintenance effort and toxic battery waste. 

ubiquitous


 


Ideally, we want wireless sensing nodes to be operate self-sustainbly to sense diverse set of 
While ideally we would wants systesm to be self-sustaianble in all scenrios, this is 




This requires the hardware system to be embedded in everyday objects and surfaces without being an obstacle for its usage or aesthetics and self-sustainable to avoid constant battery maintenance effort and toxic battery waste. 

This is a hard research problem -- 
1. the power sources available for everyday objects like tables, sofa or wall are less than a uW of power. 






Humans are mobile sources of energy \cite{}. Everyday human activities dissipate energy from the human body into the physical surface being interacted with -- high intensity mobile activities (10W) e.g. running release energy into the floor, medium energy (1W) e.g. walking, sitting up releases energy into shoes or sofa respectively 
, and low-power implicit activities like touch, sliding of hand  


Due to energy harvesting design constraints usually the efficiency of conversion is only 10-50%  

objects and surfaces

Every human action dissipates energy from the human body into the envir, be it high-intensity mobile activities \cite{} (e.g. running, climbing), medium energy (e.g. walking, sitting\cite{}) or low power activities like swiping/sliding, holding, touching, tapping, talking. 

Several sensing systems have been built for 

1. activity > interaction 

2. [ context sensing, input controls]

3. sensors are externally powered. 

4. recently self-sustainable sensing but they usually use high and medium intensity activities have been used--- write reasons which 

5. Low activities sensing ignored -- 
a.Consumption -- appropriate system architecture not approporiated makde which can detect such low power activities since communication is >>> power than harvested 
b. Generation -- "micro-interaction power harvesting we need proper form factor of harvetsors is VERY imp."  --  micro-interaction 

6. 


Human activity recognition sensing developed . thery require power souce. 

Human body is a heat engine which produces in ranges of XYZ uW --  of power. 
High intesity 
Middle intensity 
Low intensity 

Energy harvesting has been explored -- Humans from everyday activities also dissipate energy e.i. rotating, sliding, human speech. 


Every interaction human produce energy. Whether its intense 
interaction --> action. 





%Imagine a future where objects and surfaces in a room can be augmented with stickers which can provide information about the human presence and their interaction with the environment (e.g. door, thermostat, lights, plants, smart-home control). Embodiment of computers \cite{} in everyday physical world has been a long standing research goal \cite{}. 
%It has the potential of improving contextual sensing application by providing granular data, create diverse accessible options for controlling the smart physical environment, and tracking activities (to-do lists, on/off device). Designing such physically embedded systems requires looking at the hardware architecture with \textit{material driven sensibilities} while not compromising on the user experience or the functionality.  

We provide general architecture for wirelessly sensing fuctionality like presence (0/1), ID (multiple bits), acoustic 


 Of course, human environments are
incredibly diverse, with potentially hundreds of facets that
would be valuable to feed into intelligent systems that could
enhance everyday tasks.



% Simultaneous detection backscatter 
% Nano-Watt 
% form factor 

%Design space 
%% Perpetual sensing : photodiode, 
%% Micro-interaction powered --Thermal, TENG   



%%%% MAKE POWER EXPLORATION scenarions in ROOM. 
%%%%% characterise DISTANCE 


%% simulataneous detection which is also battery free. 
%% 

%most of the self-sustainable sensing had been shown to harvest power from everyday scenarios which have power mW ranges. This requires the power source to 
% 1. not only be prolonged  or very high in impact --- walking few steps generates enough power to send out a bluetooth ping, 
% 2. but also have the right kind of power management circuitry which often makes the circuit complictated. 
% 3. being able to havest power from more generalised objects around easily. not specif objects like --  furnace, microwave, lamp... but generic surfaces of the room. 


%%ambient environemnt/implict activities/micro-interactions  -- standard environemnt there is power generation which is very amobient, speeech, himan motion, sitting sliding 
%% make caterories of activities which are like that. 

% ENERGY HARVESTING FROM AMBIENT ENVIRONMENT. 
%human activites are in nW. which makes it hard to build self-sustainable sensing node. 
% sliding /tap/ touching generate/ 
%% speech. 
%tool  and heater/flow infrastructure generate mW-W of power. 

%Biomedical energy harvestors 

% book sliding scenario. 
%subtle interaction 




%============================================
%============================================
%============================================
%MEETING NOTES ================================



There are variety of batteryfree simple switches that you can buy commercially. Whats the downside of it? they have bulky form factor because that's needed in order to be able to harvest to do the communication, these things do not have a paper like form factor and something to argue that it would be nice to have[put on objects]. and the biggest problem is power. the threshold of power needed to communicate something 


So in this paper is going to show is to do some novel simple circuitry , which is very low power but also done in such a way that you can make them thin and have an appropriate form factor. 

We have had these self-sustainable switches , limitation is the form factor the kind of interactions and the amount of power, so we would like it to be thin , recieve different kinds of inputs from all different kinds of people ...but we cannot do that because the power required to something communicate the barrier. So we are gonna show you, a way to produce a very low power submicrowatt capability to sense a wide variety of interactions and communicate them in indoor office setting within range of RF infrastructure. 

making interfaces for indoor office 

We want to provide "thin form factor self-sustainable switches" . its an advance on battery free communicating devices. 


Enocean self-powered switches are inteseting, but they are limited in to 
push interactions -- touch, slides lot lesser/easier in input power.
bulky form factor -- these things look like flex circuit
ID --    more rich in information it can do presence, direction/speed sensing, audio 
 
expand range of input interactions 
RICHER INPUT : interactions of both input which can control  
(presence - touch , ID - slides , audio) --
not limited to pressing a button, and pressing a button hard. 

rich power sources : light, vibration, heat 
and they have different situations where they are useful 


This will enable far wider range of human interaction for far wider range of people
(because you do not require much physical effort to do)

 
Keeping power as main factor several 
-- the \textit{operational power budget} required to communicate the required input-control information (e.g. touch, speech), 
-- the selection of appropriate \textit{power harvesting technique} which is sufficient to power the system  dictates the form factor . 

For example, with traditional digital active communication the power requirement is so high (mW) that no human-powered technique is enough communicate any usable information based on simple light touches. 


They are all low enough power that its practical to be able to power to provide the power needed either by a separate harvester or the phenomenon of interaction itself 

You can create simple human interactions in a way that it can be placed in a range of TX/RX 

argument of form factor mixed with simple circuitry. 
Simple circuitry not simply manufactored  --- 


nW power oscillators being in put in terms of interaction sensing. previous examples are in 50 uW 




Types of indoor environment
kitchen, 
bedroom, studyroom, living room, tv room,
auditorium, 
game controller 




Discussion 

1. here is a way for leveraging subthreshold electronics for interesting User interface stuff without having batteries or wired infrastructure 

2. Mike's transistors -- The form factor is not as compelling as we want yet but there is new technology which is coming, which 





Touch 
--- single finger or hand   -- presence of human on sofa, opening a drawer, game controller | together 
--- multiple discrete touch (4) -- simple keypad/remote --polling, poster feedback in a conference room  | separate 

Gesture 
--- Swipe  -- direction left/right swipe/speed : books from shelf, music/thermostat control | together
--- send a unique ID | together

Audio 
--- SATURN (alexa).  --extended microphone in a conference room, input for smart home control | separate 





%============================================
%============================================
%============================================
%OLD INTRO ============================================

%LIMITATIONS OF COMMERCIAL BATTERY-FREE SWITCHES: 
%NOTE : I HAVE WRITTEN THE BELOW BULLET POINTS IN SHORT below 
%\begin{itemize}
%\item \textbf{Limited in input interaction possibilities:} The switches is operated through a push of a hand, which moves a magnet between coils resulting in micro-generation of power due to electromagnetic induction effect which in-turn communicates an ID to an indoor central hub. Due to the way power is generated, the switch interaction is limited to a single input method i.e. explicit push of a hand. This restricts the population who can operate the switch, e.g children or elderly may find it hard to operate. This also limits the application opportunities where the switch can be deployed e.g., implicit human activities like touch of a hand which conveys presence of a human are excluded. 
%\item \textbf{Power threshold is enough to only communicate  ID:} With the amount of power harvested from a single push the information communicated by the switch is confined to a unique ID, which restricts the application scenarios to a ping or toggle e.g, light switch on/off, and scenarios where multiple choice selection is require e.g, polling, direction selection are not possible. Creation of such scenarios would require deployment of multiple of these buttons resulting in increase of both cost and space for deployment. In addition, rich inputs like speech are completely out of bounds because of limited power budget. 
%\item \textbf{Bulky in form factor:} The coil and magnets required for power generation make the form factor bulky, which limits the places the switch can be mounted e.g., everyday objects. 
%\item \textbf{Complex Circuitry:} The switch circuit consists of a power management IC and a digital micro-controller which results in higher consumption of power and complicates the circuitry. 
%\end{itemize}





touch : presnece detection, 

The blurring of our physical and digital lives has resulted in the rise in demand for granular data about our environment and how we interact with it.  
Researchers have pushed for finding creative ways for deployment of the sensing nodes in our everyday physical spaces for finer context sensing and accessible input control applications. 
One of the ways is to directly instrument the sensing node onto the objects and surfaces itself for context sensing and accessible input control applications.
With main focus on form factor as the system design parameter, such solutions are often tethered to a power source, limiting their placement in the indoor setting, or require battery for operation which results in both maintenance effort and toxic waste generation. 
There has been recent push for self-sustainable batteryless wireless sensing system architectures where the sensing node is powered by the ambient power sources. 
Since the power required by these wireless sensing nodes for operation and active communication is 2mW-10mW depending on the type of data being communicated, these can only be powered by high energy power source with prolonged energy generation e.g. Human walking, electrical equipment like mixer, room heater. To reduce the power consumption for a wireless sensing node t 

and above 50uW for backscatter communication,

Form factor : without being a hindrance to the object's functional usage or aesthetics

With the design parameter of 

%to detect direct interactions without being a hindrance to the object's functional usage or aesthetics
%

In an ideal scenario of true ubiquitous interaction sensing; the sensing node should be embedded or instrumented onto everyday objects itself to detect direct interactions without being a hindrance to the object's functional usage or aesthetics, with multiple of such smart objects in the environment they should be battery-free in other words self-sustainable in their operation in order to avoid constant battery maintenance or toxic waste. 




Achieving true ubiquitous interaction sensing for context sensing and accessible input control applications requires the sensing node to be :  
\begin{itemize}
    \item Embedded in everyday surfaces without being a hindrance in the object's functional usage or aesthetics, 
    \item Self-sustainable to avoid constant battery maintenance or toxic waste and, 
    \item Low in its circuit complexity e.i without expensive micro-controllers or power management IC to effectively limit the cost.  
\end{itemize}
In addition to full-filling above listed design parameters the sensing should not compromise on its functional usage --e.g.. richness of information sensed (e.g, on/off, ID, audio), simultaneous operation of multiple of sensing nodes, decent range of sensing for practical applications. Balance between all the requirements is a hard research problem to solve because: 




The practical sources of power harvesting For a wireless sensing nodes embedded in surface are limited to omnipresent electromagnetic waves (e.g., light and RF) or in-situ power generated from human micro-interactions with the object.   

Critical factor for self-sustainable system operation for a surface embedded wireless nodes is that the input power harvested from the ambient sources or human's micro-interaction should be more or equal to the power required for the functional operation. 





1. With the blurring of our digital and physical lives, there has been a constant push towards finding how humans interact with their everyday surroundings for granular context sensing and  accessible input controls. 

2.Humans are mobile sources of mechanical and thermal energy \cite{}. The human body dissipate varied magnitudes of power for different activities and interactions e.g., high mobility activities like running utilize 100 Watts of human body power, medium energy activities like walking and sitting up generate several 10's W of power, on the other hand, low energy micro-interactions like touching with a finger(keystroke), hand swiping over a surface are orders of magnitude lower, only 10-100 milliWatts of power\cite{}.
 
3. Extensive research on building sensing and power harvesting systems for high and medium powered human activities have demonstrated that only fraction (0.01-1\%) of the energy dissipated from the body can be practically harvested from the surfaces with which interact with. e.g power for walking is 67W but only 1.5mW/step can be practically harvested from the shoes \cite{}. This is majorly because of the power losses from energy device employed, the transducer phenomenon selected, **form factor** and the power management circuit. 
%(1.3*0.001)/67*100
% thermal -- 4cm2/(1.9*100*100)cm2=0.0002 ratio of body are of finger. 
% 2
4. Consequently, even with one of the best power harvest low power micro-interaction activities can practically harvested only micro watts of power \cite{}. Add with that the form factor 

This power barrier has been limiting 

With current much power till now has been majorly used only for sensing purpose. 

 
 
 
 
 
 
 
 
 
 
 
 
 
 %There is a trade-off between the above four design parameters, and accomplishing  all of them together for the whole system is a challenging research challenge. With the increase in the functionality of the wireless sensor (e.g. sampling rate, information bit rate, range), both the circuit complexity, power increases. One common technique to lower them is shift from digital towards analog circuitry 
%and second is move the active radio to generation 
%When the power increases, if the amount of energy that can be harvested from the maintenance-free operation in such cases, 
%the harvester size (more photo-diode, thermo-electric are), thickness (using electromagnetic harvesters with coils and magnets) , complexity of the power management ( increased.  


%e.g. in battery-free switches like enocean, When the power increases, it is not just the 

%To keep the maintenance-free operation in such cases, significant work has been done build 

%If the power goes beyond 50uW the energy harvester and power management required is too large/thick/heavy with general ambient indoor power sources , resulting 

%In this paper, we focus on finding the sweet spot between the four design parameters. 

%reduction of power to nano-watt range with  while keeping the functionality of wireless sensing. This has 

%There have been several works in the HCI community that have focuses on flexible sensing, but are often occom 



==> old_theory_of_operation.tex <==
\section{Theory of Operation : WILL SHIFT TO RELATED WORK--NEED SOME TIME--ON IT}
% There are two main electrical phenomena which enable the nano-watt power budget of our system. The first factor is a special type of transistor which has a zero threshold voltage. This transistor type enables a ultra low startup voltage for our MARS tag ($\startupVoltage$ mV) \cite{junior2012zero}. The enabling phenomenon is the Frequency Shifted (FS) analog backscatter communication technique. This FS technique has gained much popularity in the system and networking research domain in the last decade, due to its promise for maintenance-free distributed sensing \cite{xu2018practical}. Individually, neither the use of Zero $V_{th}$ transistor in circuits nor the FS backscatter are new concepts. The combination of both of these techniques together however lends novelty to our paper. 

%\subsection{\textbf{Zero-Threshold Voltage MOSFET to enable ultra-low Supply Voltage}} The MOSFET is a three terminal device (gate, source and drain) which forms a basis for modern electronics. Each MOSFET device has a threshold voltage, $V_{TH}$, which is determined by the manufacturing process. This threshold voltage, $V_{TH}$, is the minimum amount of voltage applied to the gate needed to create a conducting path between the MOSFET's source and drain terminals. Typically a MOSFET requires a supply voltage, $V_{DD}$, which is a few 100's mV higher than $V_{TH}$. This difference between $V_{DD}$ and $V_{TH}$ is called the gate overdrive. As the feature size in modern MOSFET devices scales down (Moore's Law \cite{schaller1997moore}),  the required $V_{DD}$ decreases, but the $V_{TH}$ does not scale down with equal proportion \cite{gonzalez1997supply}. This becomes important in the context of circuit power requirements which are often a critical concern for hardware designers and applications researchers. Overall device power requirement relates quadratically to the $V_{DD}$. One way to lower the circuit power consumption is to lower the $V_{DD}$.  If  however the $V_{DD}$ is lowered too much, it degrades the performance of the circuit due to the diminished gate overdrive. A potential work around to maintain the performance with lower supply voltage is to reduce threshold voltage, $V_{TH}$ so as to maintain adequate gate overdrive. 

%\begin{center}
%\begin{figure}[!ht]
%\includegraphics[width=12cm]{samples/Figures/2.1_theory_of_operation_vth.png}
%\caption{\textbf{Theory of Operation : Zero-$V_{th}$ Transistor} A. zero threshold voltage transistor have higher current drive capability in comparison to low threshold and conventional transistors. \cite{junior2012zero} B. Region of operation of zero threshold voltage transistor \cite{ALD110800} exploited in our MARS system architecture } 
%\label{fig:theory_of_operation_zero_vth}
%\end{figure}
%\end{center}
%\vspace{-0.4in}

%Zero-$V_{TH}$ MOSFETs were introduced in the mid 90's \cite{burr1994200} and it was soon realised that these transistors had exponential increase in sub-threshold current \cite{macii2004ultra}. \autoref{fig:theory_of_operation_zero_vth}  shows a Zero-$V_{TH}$ transistor (green) which has a three orders of magnitude higher current consumption than a standard transistor (red). Since the devices are always on due to  0V $V_{TH}$ this means they consume significantly high leakage power\cite{gonzalez1997supply}.  Thus Zero-$V_{TH}$ MOSFETs were never received much acceptance in the hardware community. Alternatives were explored with low-$V_{TH}$ ($\sim 300$ mV) devices, which were more appropriate for their trade-off between low-supply voltage (active power) and leakage current (leakage power) (\autoref{fig:theory_of_operation_zero_vth}a orange). 


%Recently,  by leveraging floating gate MOSFET design \cite{seo2004low} and EPAD technology \cite{EPAD}, manufacturers like Advanced linear Devices have been able to reduce $V_{TH}$ to $\sim$ 10 mV e.g ALD110800A \cite{ALD110800} while still maintaining leakage current to be $\sim 1uW$. This results in extremely low-supply voltage like \startupVoltage mV becoming practical for circuits. These novel near Zero-$V_{TH}$ transistors, often colloquially still referred to as Zero-$V_{TH}$ transistors hold a great potential for nano-powered analog and RF-systems. The region marked in (\autoref{fig:theory_of_operation_zero_vth}b) shows a voltage range of +/- 0.15V and current $<5 uA$. In our paper we exploit this region to build an ultra-low startup power oscillator which consumes just $500 nW$ up to $1 MHz$ operation frequency.


%\subsection{\textbf{Frequency Shifted Analog Backscatter Communication}}
%Since the concept of modulating Radio Frequency (RF) for communication was proposed in 1948 \cite{stockman1948communication}, a considerable amount of research and development has been conducted in building wireless systems. One such specific communication technique is called \textit{backscatter}, which literally means reflection. In this technique, a specifically designed and tuned tag which senses information is illuminated with RF waves. The tag modulates a property of the incident RF waves (e.g amplitude, frequency, phase) according to sensed information and reflects it back. One of the earliest examples of backscatter, is The Thing (also commonly refereed to as the Great Seal bug) built by Leon Theremin \cite{brooker2013lev}. Both analog and digital techniques can be utilized to modulate the incident RF waves in backscatter communication devices. While digital backscatter communication (e.g. RFID \cite{}) is generally considered more robust, analog communication is an order of magnitude lower in power budget, simpler in circuitry, and supports rich sensing \cite{}. Analog backscatter transmissions are typically noisy because the data is sent on the same channel as the carrier signal. This can be avoided if the backscatter tag isolates its spectrum by shifting itself to an adjacent non-overlapping frequency band \cite{} (\autoref{fig:fs-backscatter}). This Frequency shift (FS) based analog backscatter technique has levels of noise tolerance comparable to digital systems while still maintaining the benefits of analog circuitry.  Due to these advantages we have employed FS-backscatter in our MARS system architecture.  



%\begin{center}
%\begin{figure}[!ht]
%\includegraphics[width=14cm]{samples/Figures/2.1_theory_of_operation_backscatter.png}
%\caption{ \textbf{Theory of Operation : Frequency Shifted Analog Backscatter Communication} MARS System Architecture consisting of Transmitter, Receiver and multiple MARS tags in the environment. Transmitter produces UHF RF Non-modulated continuous carrier wave (yellow) which is incident on the tags. Each MARS tag consists of an ultra-low-power oscillator, oscillating at a particular frequency ( e.g., Tag 1 oscillates at F1 frequency). The input interactions result in change in electrical property (blue) resulting in frequency modulating the oscillator signal (magenta). This signal is backscattered  to the receiver (green) using analog impedance switch and antenna. The receiver, receives frequency modulated information at different bands from each tag which is demodulated back to the original sensed signal.} 
%\label{fig:fs-backscatter}
%\end{figure}
%\vspace{-0.4in}
%\end{center}  


%The advent of the Internet of Things generation, has created smart objects (e.g., smart home control, thermostats, light control, fridge) that can interact with humans or connect with other devices through the internet. While these smart devices are specifically factory manufactured and require regular battery maintenance, there is another category of already existing everyday artifacts that do not the capability to connect the environment or sense human interactions. 

==> reciever.tex <==
\subsection{Transceiver Processing} 
The radio frequency transceiver utilized in this work is based around the Etteus N210 USRP software defined radio (SDR) and the GNURadio-Companion (GRC) software suite. 

Four software processing flow graphs were developed in GRC which handle both transmitting the CW power signal to the sensor tags as well as receiving backscattered signals and conducting digital signal processing to decode data from the backscattered signals. 

Each GRC flow graph is optimized for a particular modality of backscattered signal but they all share a similar set of initial digital signal processing steps: SDR signal source, low pass filter, frequency translation. As displayed in figure (insert figure), immediately after the digital samples are received from the SDR, a low pass filter is applied to eliminate high frequency noise and throw away a large section of signal bandwidth which does not contain the backscattered signals of interest. 

This initial low pass filter for cutting signal bandwidth reduces the amount of aliasing which will occur downstream in the processing pipeline when re-sampling is applied. Next, a frequency translation step is applied to shift the backscattered signal (typical offset from the 915MHz carrier by between 200 and 700KHz) down to 0Hz offset. 

The translation to 0Hz offset allows further signal filtering, demodulation, and down sampling. In the cases where frequency shift keying (FSK) is the modality of backscattered signal, no additional demodulation is required in the signal processing pipeline. 

For frequency modulated (FM) signals, a Wide Band Frequency Modulation (WBFM) demodulation block is utilized to separate the backscattered signal from the backscattered carrier wave. Finally, these processed signals are downsampled into the audible region at a rate of 48KHz using a rational resampler block. 


\subsection{Swipe based Direction sensing }
%%Chad transceiver section for SATURN audio%%
The MARS facilitated capacitive swipe based direction sensing processing implementation involves both the gnuradio pipeline outlined above as well as an additional python signal processing pipeline. The transmission is handled by two blocks in GRC: 100Hz sine wave signal source is fed into a USRP sink block tuned to 915MHz at 1MHz sample rate. Back scattered signal reception and processing are handled simultaneously in the same flow graph as the transmission processing. For reception, a USRP source block is tuned to receive signals at 915MHz with a 1MHz sample rate. Immediately after the USRP source block, a frequency translating FIR filter is applied to shift the backscattered swipe signal from its 330KHz offset frequency to 0Hz, low pass filter the signal shifted to 0Hz with a 30KHz low pass cutoff, and to decimate by a factor of 10. Next a zeromq tcp publisher block is utilized to transmit the swipe signal samples from GRC to python. In a corresponding python program which runs simultaneously with the GRC flowgrpah, a zeromq subscription is initiated with the publisher implemented in the GRC flowgraph. The python program receives complex-64 formatted signal samples via the zeromq subscription and stores them in a numpy array. Once the numpy array is filled, the python program uses the numpy fft library to compute the fast Fourier transform (FFT) on the raw signal. Once the raw signal has been transformed via the FFT, an argmax is computed on the resultant 2D array across the time axis to construct a 1D array with each time step containing the frequency of highest intensity at that time step. This 1D array is then smoothed with a 100x100 mean kernel to reduce noise. After the smoothing step, the minimum and maximum values of the signal are found and a linear regression is plotted between those points. The slope of this linear regression corresponds to the direction of the swipe.  



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Swipe based Unique ID }
%%Chad transceiver section for SATURN audio%%
The MARS facilitated capacitive swipe based unique ID transmission sensing processing implementation involves both the gnuradio pipeline outlined above as well as an additional python signal processing pipeline. The transmission is handled by two blocks in GRC: 100Hz sine wave signal source is fed into a USRP sink block tuned to 915MHz at 1MHz sample rate. Back scattered signal reception and processing are handled simultaneously in the same flow graph as the transmission processing. For reception, a USRP source block is tuned to receive signals at 915MHz with a 1MHz sample rate. Immediately after the USRP source block, a frequency translating FIR filter is applied to shift the backscattered swipe signal from its 330KHz offset frequency to 0Hz, low pass filter the signal shifted to 0Hz with a 30KHz low pass cutoff, and to decimate by a factor of 10. Next a zeromq tcp publisher block is utilized to transmit the swipe signal samples from GRC to python.

In a corresponding python program which runs simultaneously with the GRC flowgrpah, a zeromq subscription is initiated with the publisher implemented in the GRC flowgraph. The python program receives complex-64 formatted signal samples via the zeromq subscription and stores them in a numpy array. Once the numpy array is filled, the python program uses the numpy fft library to compute the fast Fourier transform (FFT) on the raw signal. Once the raw signal has been transformed via the FFT, an argmax is computed on the resultant 2D array across the time axis to construct a 1D array with each time step containing the frequency of highest intensity at that time step. This 1D array is then smoothed with a 100x100 mean kernel to reduce noise. After the smoothing step, the signal is prepared for pattern matching with dynamic time warping (DTW). This DTW based pattern matching was not considered to be within the scope of this current publication but can be developed in future works.   


\subsection{Speech }
touch and send audio. 
%%Chad transceiver section for SATURN audio%%
The speech transceiver processing implementation for MARS facilitated SATURN audio exactly follows the architecture outlined in the above transceiver processing section. The transmission is handled by two blocks in GRC: 100Hz sine wave signal source is fed into a USRP sink  block tuned to 915MHz at 2MHz sample rate. Back scattered signal reception and processing are handled simultaneously in the same flow graph as the transmission processing. For reception, a USRP source block is tuned to receive signals at 915MHz with a 2MHz sample rate. Immediately after the USRP source block, a frequency translating FIR filter is applied to shift the backscattered frequency modulated audio signal from its 670KHz offset frequency to 0Hz, band pass the signal shifted to 0Hz with a 60Hz high pass and a 4KHz low pass, and to decimate by a factor of 10. Next a wide band frequency modulated demodulation block is applied to demodulate the modulated audio signal. To the demodulated audio signal a rational resampler block is applied to reduce the sample rate to 48KHz and a multiply constant block is applied to increase the amplitude of the audio signal. Finally the audio signal is fed into a audio sink where it is output through the transceiver computer's speakers.

\subsection{Multi-Touch / Game Controllers}
%%Chad transceiver section for SATURN audio%%
For simultaneously processing multiple touch inputs from several MARS tags, the GRC flow graph pipeline described for the previous examples is modified with additional frequency translating FIR filters. The software pipeline for multi touch detection involves three main steps: a band-pass frequency translating FIR filter to shift each MARS tag's signals to 0Hz, a set of additional band pass filters for each touch button signal from each MARS tag, a set of signal intensity threshold detectors which trigger when a high level of signal occurs within one of the band-pass filter allowed regions. After the three step flow graph process, the threshold activation's can be interfaced with external software for controlling video games or IoT devices via a TCP network socket. 
